Self-contradictory Hallucinations of Large Language Models: Evaluation, Detection and Mitigation

Large language models (large LMs) are susceptible to producing text that contains hallucinated content. An important instance of this problem is self-contradiction, where the LM generates two contradictory sentences within the same context. In this work, we present a comprehensive investigation into self-contradiction for various instruction-tuned LMs, covering evaluation, detection, and mitigation. Our primary evaluation task is open-domain text generation, but we also demonstrate the applicability of our approach to shorter question answering. Our analysis reveals the prevalence of self-contradictions, e.g., in 17.7% of all sentences produced by ChatGPT. We then propose a novel prompting-based framework designed to effectively detect and mitigate self-contradictions. Our detector achieves high accuracy, e.g., around 80% F1 score when prompting ChatGPT. The mitigation algorithm iteratively refines the generated text to remove contradictory information while preserving text fluency and informativeness. Importantly, our entire framework is applicable to black-box LMs and does not require retrieval of external knowledge. Rather, our method complements retrieval-based methods, as a large portion of self-contradictions (e.g., 35.2% for ChatGPT) cannot be verified using online text. Our approach is practically effective and has been released as a push-button tool to benefit the public at https://chatprotect.ai/.

==> figures/selfcheckgpt-contra.tex <==
% ours
\addplot [draw=mygreen, line width=1.1pt] coordinates {
        (100.0, 15.878916622411046)
        (97.32441471571906, 17.81450872359963)
        (96.65551839464884, 18.802862719583604)
        (95.65217391304348, 19.449166950017002)
        (94.98327759197325, 20.056497175141246)
        (94.81605351170569, 20.70854638422206)
        (94.48160535117057, 21.91621411947246)
        (94.31438127090301, 22.732769044740024)
        (94.14715719063545, 23.5663457513604)
        (93.81270903010034, 24.519230769230766)
        (93.64548494983278, 24.691358024691358)
        (93.47826086956522, 25.796031379787728)
        (93.31103678929766, 26.58408766079085)
        (93.1438127090301, 26.973365617433416)
        (92.97658862876254, 28.498206048180418)
        (92.80936454849498, 29.05759162303665)
        (92.47491638795987, 29.683306494900698)
        (92.3076923076923, 31.292517006802722)
        (92.14046822742475, 32.70029673590504)
        (91.9732441471572, 32.97362110311751)
        (91.80602006688964, 34.205607476635514)
        (91.63879598662207, 34.971282705807276)
        (91.47157190635451, 38.60268172194778)
        (91.30434782608695, 38.97216274089936)
        (91.1371237458194, 40.07352941176471)
        (90.3010033444816, 42.05607476635514)
        (90.13377926421404, 42.17527386541471)
        (89.96655518394648, 42.49605055292259)
        (89.79933110367892, 43.271555197421435)
        (88.96321070234113, 45.19966015293118)
        (88.79598662207357, 47.7088948787062)
        (88.62876254180601, 48.98336414048059)
        (88.46153846153845, 49.4392523364486)
        (88.2943143812709, 50.142450142450144)
        (88.12709030100334, 50.52732502396932)
        (87.95986622073578, 52.07920792079208)
        (87.79264214046822, 53.735926305015354)
        (87.45819397993311, 55.22703273495249)
        (87.29096989966555, 56.80087051142546)
        (86.95652173913044, 58.42696629213483)
        (86.62207357859532, 68.70026525198939)
        (86.45484949832776, 70.91906721536351)
        (86.12040133779264, 73.6766809728183)
        (85.95317725752508, 74.9271137026239)
        (85.78595317725753, 75.7754800590842)
        (85.61872909698997, 76.07726597325409)
        (85.45150501672241, 78.25421133231241)
        (85.28428093645485, 78.94736842105263)
        (85.11705685618729, 80.41074249605056)
        (84.94983277591973, 81.41025641025641)
        (84.78260869565217, 82.70799347471451)
        (84.61538461538461, 84.19301164725458)
        (84.44816053511705, 86.47260273972603)
        (84.2809364548495, 86.5979381443299)
        (84.11371237458194, 86.87392055267703)
        (83.94648829431438, 87.00173310225303)
        (83.77926421404682, 87.2822299651568)
        (83.4448160535117, 87.39054290718039)
        (83.27759197324414, 88.14159292035399)
        (83.11036789297658, 89.06810035842294)
        (82.94314381270902, 89.20863309352518)
        (82.77591973244147, 89.5117540687161)
        (82.6086956521739, 90.14598540145985)
        (82.44147157190636, 90.45871559633028)
        (82.2742474916388, 90.60773480662984)
        (82.10702341137124, 90.75785582255084)
        (81.93979933110369, 90.9090909090909)
        (81.77257525083613, 91.23134328358209)
        (81.43812709030101, 91.36960600375235)
        (80.76923076923077, 91.47727272727273)
        (80.43478260869566, 91.61904761904762)
        (79.26421404682274, 91.86046511627907)
        (79.09698996655518, 92.02334630350194)
        (78.26086956521739, 92.1259842519685)
        (77.92642140468227, 92.27722772277228)
        (77.25752508361204, 92.4)
        (76.08695652173914, 92.2920892494929)
        (75.91973244147158, 92.4643584521385)
        (75.75250836120402, 92.63803680981594)
        (75.58528428093646, 92.81314168377823)
        (75.08361204013379, 92.96066252587993)
        (74.91638795986621, 93.13929313929314)
        (74.08026755852842, 93.26315789473684)
        (73.57859531772574, 93.41825902335457)
        (73.07692307692307, 93.57601713062098)
        (72.90969899665552, 93.76344086021506)
        (71.57190635451505, 93.6542669584245)
        (70.23411371237458, 93.54120267260579)
        (70.06688963210702, 93.94618834080718)
        (69.56521739130434, 94.11764705882352)
        (69.06354515050167, 94.29223744292237)
        (67.89297658862876, 94.41860465116278)
        (66.5551839464883, 94.3127962085308)
        (65.21739130434783, 94.20289855072464)
        (65.05016722408027, 94.64720194647201)
        (63.7123745819398, 94.54094292803971)
        (63.37792642140469, 94.75)
        (63.21070234113713, 94.9748743718593)
        (62.70903010033445, 95.17766497461929)
        (62.374581939799334, 95.64102564102565)
        (60.70234113712375, 95.77836411609498)
        (60.200668896321076, 96.0)
        (59.36454849498328, 96.2059620596206)
        (58.52842809364549, 96.41873278236915)
        (58.026755852842804, 96.65738161559888)
        (57.859531772575245, 96.9187675070028)
        (57.52508361204013, 97.45042492917847)
        (56.020066889632105, 97.667638483965)
        (52.508361204013376, 97.81931464174455)
        (50.0, 97.7124183006536)
        (48.82943143812709, 97.98657718120806)
        (45.65217391304348, 97.84946236559139)
        (43.47826086956522, 97.74436090225564)
        (39.96655518394649, 97.95081967213115)
        (39.79933110367893, 98.34710743801654)
        (35.953177257525084, 98.17351598173516)
        (35.618729096989966, 98.61111111111111)
        (32.10702341137124, 98.46153846153847)
        (28.428093645484946, 98.83720930232558)
        (25.25083612040134, 98.69281045751634)
        (23.244147157190636, 98.58156028368793)
        (21.40468227424749, 98.46153846153847)
        (19.732441471571907, 98.33333333333333)
        (17.558528428093645, 98.13084112149532)
        (16.220735785953178, 97.97979797979798)
        (15.050167224080269, 97.82608695652173)
        (13.712374581939798, 97.61904761904762)
        (13.043478260869565, 97.5)
        (12.37458193979933, 97.36842105263158)
        (10.200668896321071, 96.82539682539682)
        (9.866220735785953, 96.72131147540983)
        (8.862876254180602, 98.14814814814815)
        (8.193979933110368, 98.0)
        (7.357859531772576, 97.77777777777777)
        (6.354515050167224, 97.43589743589743)
        (5.852842809364549, 97.22222222222221)
        (4.849498327759197, 96.66666666666667)
        (4.013377926421405, 96.0)
        (3.3444816053511706, 95.23809523809523)
        (3.177257525083612, 95.0)
        (2.341137123745819, 100.0)
        (0.8361204013377926, 100.0)
        (0.0, 100.0)
};
% BertScore
\addplot [draw=myred, line width=1.1pt] coordinates {
        (100.0, 15.032107413893753)
        (100.0, 15.089364195722238)
        (100.0, 15.11150234741784)
        (100.0, 15.115937775168769)
        (98.44660194174757, 14.995563442768411)
        (96.50485436893203, 14.880239520958083)
        (95.92233009708738, 14.983318168031543)
        (92.62135922330097, 15.085388994307399)
        (92.42718446601941, 15.188257817485642)
        (91.6504854368932, 15.289925494007125)
        (89.90291262135922, 15.155482815057283)
        (87.37864077669903, 15.045135406218657)
        (86.60194174757282, 15.149456521739129)
        (85.04854368932038, 15.025728987993139)
        (82.52427184466019, 14.907050157839356)
        (76.69902912621359, 14.805097451274364)
        (76.50485436893204, 14.907302307983352)
        (75.33980582524272, 14.80351011064479)
        (75.14563106796116, 14.907550077041604)
        (74.5631067961165, 15.017598748533437)
        (73.7864077669903, 15.121368881814565)
        (73.20388349514563, 15.019920318725099)
        (72.03883495145631, 14.917571371129876)
        (71.45631067961165, 15.020408163265305)
        (70.48543689320388, 14.870954526833266)
        (68.93203883495146, 14.754779717373234)
        (65.4368932038835, 14.639443961772372)
        (63.883495145631066, 14.74675033617212)
        (62.33009708737865, 14.624145785876994)
        (61.165048543689316, 14.482758620689657)
        (60.970873786407765, 14.591078066914498)
        (59.6116504854369, 14.696026807084731)
        (58.44660194174758, 14.590402326708677)
        (57.28155339805825, 14.474975466143277)
        (56.116504854368934, 14.363817097415508)
        (55.72815533980583, 14.465725806451612)
        (54.757281553398066, 14.358452138492872)
        (53.980582524271846, 14.227226202661209)
        (53.786407766990294, 14.330056906363167)
        (52.038834951456316, 14.217506631299734)
        (50.29126213592233, 14.106753812636166)
        (50.09708737864078, 14.20704845814978)
        (48.932038834951456, 14.101846670397315)
        (48.737864077669904, 14.204867006225241)
        (47.96116504854369, 14.090131203650886)
        (47.76699029126213, 14.26086956521739)
        (47.57281553398058, 14.369501466275661)
        (47.18446601941748, 14.472900536033354)
        (46.40776699029126, 14.345738295318128)
        (46.213592233009706, 14.450516089860352)
        (45.8252427184466, 14.558914250462676)
        (44.85436893203884, 14.4375)
        (44.46601941747573, 14.330413016270338)
        (44.07766990291262, 14.223057644110277)
        (43.30097087378641, 14.113924050632912)
        (42.71844660194174, 14.221073044602456)
        (41.16504854368932, 14.324324324324325)
        (40.3883495145631, 14.21736158578264)
        (38.640776699029125, 14.326853851691865)
        (37.86407766990291, 14.22319474835886)
        (37.4757281553398, 14.118507681053401)
        (37.28155339805825, 14.232765011119348)
        (36.699029126213595, 14.093959731543624)
        (36.50485436893204, 14.242424242424242)
        (36.310679611650485, 14.351496546431312)
        (34.75728155339806, 14.139020537124802)
        (34.1747572815534, 14.035087719298245)
        (33.78640776699029, 14.146341463414632)
        (33.398058252427184, 14.040816326530612)
        (33.20388349514563, 14.1439205955335)
        (33.00970873786408, 14.249790444258172)
        (32.81553398058252, 14.358538657604077)
        (32.42718446601941, 14.45887445887446)
        (32.23300970873787, 14.561403508771932)
        (31.2621359223301, 14.42652329749104)
        (31.06796116504854, 14.532243415077204)
        (30.679611650485437, 14.389799635701275)
        (29.902912621359224, 14.25925925925926)
        (29.514563106796114, 14.152700186219738)
        (29.320388349514566, 14.367269267364415)
        (27.766990291262132, 14.200595829195631)
        (27.378640776699033, 14.31472081218274)
        (26.990291262135923, 14.212678936605316)
        (26.601941747572816, 14.080164439876668)
        (26.21359223300971, 13.946280991735538)
        (25.8252427184466, 13.811007268951196)
        (25.436893203883493, 13.702928870292888)
        (24.854368932038835, 13.588110403397028)
        (24.466019417475728, 13.475935828877006)
        (24.271844660194176, 13.586956521739129)
        (23.883495145631066, 13.472070098576122)
        (23.300970873786408, 13.348164627363737)
        (23.106796116504853, 13.461538461538462)
        (22.330097087378643, 13.294797687861271)
        (22.135922330097088, 13.396004700352526)
        (21.941747572815533, 13.598074608904934)
        (21.74757281553398, 13.708690330477355)
        (21.553398058252426, 13.602941176470587)
        (21.35922330097087, 13.715710723192021)
        (20.97087378640777, 13.55081555834379)
        (20.776699029126213, 13.665389527458494)
        (20.19417475728155, 13.488975356679637)
        (20.0, 14.071038251366119)
        (19.41747572815534, 13.869625520110956)
        (19.02912621359223, 13.725490196078432)
        (18.446601941747574, 13.590844062947067)
        (18.25242718446602, 14.050822122571002)
        (17.475728155339805, 13.740458015267176)
        (16.893203883495143, 13.636363636363635)
        (16.699029126213592, 13.500784929356357)
        (16.310679611650485, 13.291139240506327)
        (16.116504854368934, 13.408723747980615)
        (15.922330097087379, 13.509060955518946)
        (15.728155339805824, 13.61344537815126)
        (15.339805825242719, 13.504273504273504)
        (15.145631067961165, 13.756613756613756)
        (14.951456310679612, 14.076782449725778)
        (14.757281553398057, 14.17910447761194)
        (14.563106796116504, 14.04494382022472)
        (14.36893203883495, 14.396887159533073)
        (14.174757281553399, 14.512922465208748)
        (13.980582524271846, 14.634146341463413)
        (13.78640776699029, 14.760914760914762)
        (13.592233009708737, 14.583333333333334)
        (13.398058252427184, 14.712153518123666)
        (13.203883495145632, 14.814814814814813)
        (12.815533980582524, 14.634146341463413)
        (12.62135922330097, 15.625)
        (12.427184466019417, 16.08040201005025)
        (12.233009708737864, 16.195372750642672)
        (12.03883495145631, 16.358839050131927)
        (11.844660194174757, 16.666666666666664)
        (11.650485436893204, 16.80672268907563)
        (11.45631067961165, 17.404129793510325)
        (11.262135922330096, 17.261904761904763)
        (11.067961165048544, 17.484662576687114)
        (10.87378640776699, 17.23076923076923)
        (10.679611650485436, 16.97530864197531)
        (10.485436893203884, 17.197452229299362)
        (10.29126213592233, 17.320261437908496)
        (10.097087378640776, 17.449664429530202)
        (9.902912621359224, 17.22972972972973)
        (9.70873786407767, 17.064846416382252)
        (9.514563106796116, 18.49056603773585)
        (9.12621359223301, 18.146718146718147)
        (8.932038834951456, 18.69918699186992)
        (8.737864077669903, 18.367346938775512)
        (8.54368932038835, 18.25726141078838)
        (8.349514563106796, 17.916666666666668)
        (8.155339805825243, 17.796610169491526)
        (7.961165048543689, 17.59656652360515)
        (7.766990291262135, 18.181818181818183)
        (7.572815533980583, 18.30985915492958)
        (7.3786407766990285, 18.009478672985782)
        (7.184466019417475, 17.703349282296653)
        (6.990291262135923, 17.391304347826086)
        (6.796116504854369, 18.229166666666664)
        (6.601941747572816, 18.478260869565215)
        (6.407766990291262, 18.13186813186813)
        (6.213592233009709, 17.77777777777778)
        (6.019417475728155, 18.902439024390244)
        (5.825242718446602, 19.480519480519483)
        (5.631067961165048, 19.205298013245034)
        (5.436893203883495, 19.047619047619047)
        (5.242718446601942, 18.88111888111888)
        (5.048543689320388, 19.402985074626866)
        (4.854368932038835, 19.68503937007874)
        (4.660194174757281, 19.2)
        (4.466019417475728, 21.69811320754717)
        (4.271844660194175, 22.448979591836736)
        (4.077669902912621, 27.27272727272727)
        (3.8834951456310676, 27.027027027027028)
        (3.6893203883495143, 29.6875)
        (3.1067961165048543, 27.586206896551722)
        (2.912621359223301, 33.33333333333333)
        (2.7184466019417477, 32.55813953488372)
        (2.524271844660194, 34.21052631578947)
        (2.3300970873786406, 48.0)
        (2.1359223300970873, 68.75)
        (1.9417475728155338, 66.66666666666666)
        (1.7475728155339807, 69.23076923076923)
        (1.5533980582524272, 72.72727272727273)
        (0.0, 100.0)
};
% MQAG
\addplot [draw=myblue, line width=1.1pt] coordinates {
        (100.0, 15.093205051112445)
        (100.0, 15.097744360902254)
        (100.0, 15.10228640192539)
        (100.0, 15.106831176647608)
        (100.0, 15.111378687537627)
        (100.0, 15.11592893706715)
        (100.0, 15.120481927710843)
        (100.0, 15.125037661946369)
        (100.0, 15.12959614225437)
        (100.0, 15.134157371118482)
        (99.60159362549801, 15.234613040828762)
        (99.20318725099602, 15.337234370187867)
        (99.00398406374502, 15.439577508543026)
        (98.80478087649402, 15.543716703227828)
        (98.60557768924303, 15.644753476611884)
        (98.40637450199203, 15.7475294867708)
        (98.20717131474103, 15.85209003215434)
        (98.00796812749005, 16.03650586701434)
        (97.80876494023904, 16.146004603748768)
        (97.60956175298804, 16.246684350132625)
        (95.61752988047809, 16.348773841961854)
        (95.4183266932271, 16.454826520096187)
        (94.02390438247012, 16.555594528235705)
        (93.82470119521913, 16.666666666666664)
        (92.62948207171314, 16.76884240894338)
        (92.43027888446214, 17.223459539717894)
        (92.23107569721115, 17.44536548605878)
        (92.03187250996015, 17.546524876566654)
        (89.04382470119522, 17.647058823529413)
        (88.84462151394422, 17.747711898129726)
        (88.64541832669323, 17.849979943842758)
        (87.84860557768924, 17.95602605863192)
        (87.64940239043824, 18.0623973727422)
        (87.45019920318725, 18.163011998345056)
        (87.25099601593625, 18.47321805145508)
        (85.85657370517929, 18.57758620689655)
        (85.65737051792829, 18.679409209383145)
        (85.2589641434263, 18.780166739798158)
        (85.0597609561753, 18.885448916408667)
        (84.86055776892431, 18.99242086491306)
        (84.4621513944223, 19.0990990990991)
        (84.26294820717132, 19.574271170754283)
        (84.06374501992032, 19.682835820895523)
        (83.86454183266933, 19.783834586466163)
        (83.66533864541833, 19.886363636363637)
        (83.46613545816733, 20.086289549376797)
        (83.26693227091634, 20.193236714975846)
        (83.06772908366534, 20.30185004868549)
        (81.87250996015936, 20.407149950347566)
        (81.07569721115537, 20.514112903225808)
        (80.0796812749004, 20.615384615384617)
        (79.8804780876494, 20.723514211886304)
        (79.6812749003984, 20.833333333333336)
        (79.08366533864542, 20.938818565400844)
        (78.68525896414343, 21.044219499200853)
        (78.28685258964143, 21.15177610333692)
        (78.08764940239044, 21.281216069489687)
        (77.88844621513944, 21.38949671772429)
        (77.68924302788844, 21.499448732083792)
        (77.09163346613546, 21.608040201005025)
        (76.89243027888446, 21.70978627671541)
        (76.69322709163346, 21.813031161473088)
        (75.4980079681275, 21.920185078079815)
        (75.2988047808765, 22.183098591549296)
        (74.9003984063745, 22.28808535862478)
        (74.7011952191235, 22.401433691756274)
        (74.5019920318725, 22.503008423586042)
        (73.30677290836654, 22.38442822384428)
        (73.10756972111554, 22.487745098039216)
        (72.50996015936255, 22.594661700806952)
        (72.31075697211156, 22.70168855534709)
        (71.71314741035857, 22.58469259723965)
        (71.51394422310757, 22.692793931731988)
        (70.5179282868526, 22.794591113972956)
        (70.3187250996016, 22.90720311486048)
        (69.9203187250996, 23.016393442622952)
        (69.7211155378486, 23.11756935270806)
        (69.52191235059762, 23.266666666666666)
        (69.32270916334662, 23.52941176470588)
        (69.12350597609563, 23.637602179836513)
        (68.92430278884463, 23.74742621825669)
        (68.72509960159363, 23.858921161825727)
        (67.33067729083665, 23.719298245614034)
        (67.13147410358566, 23.883770375620127)
        (66.33466135458167, 23.991354466858787)
        (66.13545816733067, 24.092888243831638)
        (65.93625498007968, 24.249084249084248)
        (65.73705179282868, 24.40828402366864)
        (65.5378486055777, 24.51564828614009)
        (65.33864541832669, 24.624624624624623)
        (64.9402390438247, 24.51127819548872)
        (64.5418326693227, 24.620060790273556)
        (64.34262948207171, 24.807987711213517)
        (64.14342629482071, 25.058365758754864)
        (63.745019920318725, 25.177025963808024)
        (63.54581673306773, 25.277337559429476)
        (63.34661354581673, 25.41966426858513)
        (63.147410358565736, 25.730519480519483)
        (62.94820717131474, 25.901639344262296)
        (62.35059760956175, 26.01828761429759)
        (61.55378486055777, 26.120033812341504)
        (60.95617529880478, 26.221079691516707)
        (60.756972111553786, 26.338514680483595)
        (60.55776892430279, 26.503923278116826)
        (60.3585657370518, 26.62565905096661)
        (60.1593625498008, 26.725663716814157)
        (59.16334661354582, 26.82926829268293)
        (58.964143426294825, 26.98268003646308)
        (58.76494023904383, 27.089072543618)
        (58.56573705179283, 27.37430167597765)
        (58.366533864541836, 27.511737089201876)
        (57.96812749003985, 27.635327635327634)
        (57.76892430278885, 27.751196172248804)
        (57.56972111553785, 27.86885245901639)
        (57.37051792828686, 27.988338192419825)
        (56.97211155378486, 28.094302554027507)
        (55.77689243027888, 28.197381671701915)
        (55.57768924302788, 28.556806550665303)
        (55.37848605577689, 28.808290155440414)
        (54.980079681274894, 28.930817610062892)
        (54.7808764940239, 29.069767441860467)
        (54.581673306772906, 29.3048128342246)
        (54.38247011952191, 29.41810344827586)
        (53.18725099601593, 29.308452250274424)
        (52.788844621513945, 29.411764705882355)
        (52.39043824701195, 29.287305122494434)
        (52.191235059760956, 29.638009049773757)
        (51.79282868525896, 29.74828375286041)
        (51.19521912350598, 29.60829493087558)
        (50.199203187250994, 29.508196721311474)
        (50.0, 29.634002361275087)
        (49.800796812749006, 29.761904761904763)
        (49.20318725099602, 29.866989117291414)
        (48.80478087649402, 29.98776009791922)
        (48.60557768924303, 30.198019801980198)
        (48.40637450199203, 30.413016270337923)
        (48.20717131474104, 30.51702395964691)
        (48.007968127490045, 30.62261753494282)
        (47.808764940239044, 30.72983354673495)
        (47.410358565737056, 30.551989730423617)
        (47.211155378486055, 30.659767141009052)
        (46.81274900398406, 30.519480519480517)
        (46.015936254980076, 30.35479632063075)
        (45.81673306772908, 30.666666666666664)
        (45.61752988047809, 30.77956989247312)
        (45.41832669322709, 31.105047748976805)
        (45.21912350597609, 31.267217630853995)
        (44.820717131474105, 31.163434903047094)
        (44.42231075697211, 30.97222222222222)
        (44.02390438247012, 31.08298171589311)
        (43.82470119521912, 31.20567375886525)
        (43.625498007968126, 31.330472103004293)
        (42.82868525896414, 31.432748538011694)
        (42.62948207171315, 31.563421828908556)
        (42.430278884462155, 31.69642857142857)
        (42.23107569721115, 31.83183183183183)
        (42.03187250996016, 31.72932330827068)
        (41.832669322709165, 31.626506024096386)
        (41.03585657370518, 31.49847094801223)
        (40.63745019920319, 31.627906976744185)
        (40.23904382470119, 31.761006289308174)
        (40.0398406374502, 31.955484896661368)
        (39.6414342629482, 31.840000000000003)
        (39.44223107569721, 32.24755700325733)
        (39.243027888446214, 32.56198347107438)
        (39.04382470119522, 32.450331125827816)
        (38.84462151394422, 32.33830845771145)
        (38.645418326693225, 32.22591362126246)
        (38.44621513944223, 32.32830820770519)
        (38.24701195219124, 32.21476510067114)
        (38.047808764940235, 32.31810490693739)
        (37.84860557768924, 32.534246575342465)
        (37.64940239043825, 32.755632582322356)
        (37.45019920318725, 32.86713286713287)
        (37.25099601593625, 32.98059964726631)
        (37.05179282868526, 33.273703041144906)
        (36.852589641434264, 33.57531760435572)
        (36.45418326693227, 33.394160583941606)
        (36.254980079681275, 33.51749539594843)
        (35.657370517928285, 33.64661654135339)
        (35.45816733067729, 33.776091081593925)
        (35.2589641434263, 33.97312859884837)
        (35.0597609561753, 34.1747572815534)
        (34.66135458167331, 33.984375)
        (34.462151394422314, 34.12228796844182)
        (34.26294820717131, 34.26294820717131)
        (34.06374501992032, 34.475806451612904)
        (33.86454183266932, 34.97942386831276)
        (33.46613545816733, 34.78260869565217)
        (33.266932270916335, 35.08403361344538)
        (33.067729083665334, 36.08695652173913)
        (32.86852589641434, 36.91275167785235)
        (32.47011952191235, 36.711711711711715)
        (32.27091633466135, 37.327188940092164)
        (31.872509960159363, 37.2093023255814)
        (31.673306772908365, 37.5)
        (31.47410358565737, 37.61904761904762)
        (31.274900398406373, 38.48039215686275)
        (31.07569721115538, 38.613861386138616)
        (30.87649402390438, 38.46153846153847)
        (30.677290836653388, 38.69346733668342)
        (30.47808764940239, 38.539042821158695)
        (30.278884462151396, 38.38383838383838)
        (30.0796812749004, 39.52879581151832)
        (29.880478087649404, 39.682539682539684)
        (29.681274900398407, 39.52254641909814)
        (29.282868525896415, 39.41018766756032)
        (29.08366533864542, 39.247311827956985)
        (28.884462151394423, 39.083557951482476)
        (28.68525896414343, 38.91891891891892)
        (28.286852589641438, 38.69209809264305)
        (27.88844621513944, 38.56749311294766)
        (27.689243027888445, 38.93557422969188)
        (27.490039840637447, 39.20454545454545)
        (27.290836653386453, 39.59537572254335)
        (27.091633466135455, 39.76608187134503)
        (26.89243027888446, 39.589442815249264)
        (26.693227091633464, 39.762611275964396)
        (26.49402390438247, 39.58333333333333)
        (26.294820717131472, 39.75903614457831)
        (26.095617529880478, 39.577039274924466)
        (25.89641434262948, 39.39393939393939)
        (25.697211155378486, 39.57055214723926)
        (25.298804780876495, 39.318885448916404)
        (25.099601593625497, 39.130434782608695)
        (24.900398406374503, 38.940809968847354)
        (24.701195219123505, 39.24050632911392)
        (24.50199203187251, 39.04761904761905)
        (24.302788844621514, 39.228295819935695)
        (24.10358565737052, 39.03225806451613)
        (23.904382470119522, 39.21568627450981)
        (23.705179282868528, 39.40397350993378)
        (23.50597609561753, 39.202657807308974)
        (23.306772908366533, 39.0)
        (23.107569721115535, 38.79598662207358)
        (22.90836653386454, 38.983050847457626)
        (22.709163346613543, 38.775510204081634)
        (22.50996015936255, 38.96551724137931)
        (22.31075697211155, 40.0)
        (22.111553784860558, 39.784946236559136)
        (21.91235059760956, 39.568345323741006)
        (21.713147410358566, 40.22140221402214)
        (21.51394422310757, 41.06463878326996)
        (21.314741035856574, 41.312741312741316)
        (21.115537848605577, 41.08527131782946)
        (20.717131474103585, 40.78431372549019)
        (20.318725099601593, 40.63745019920319)
        (20.119521912350596, 40.89068825910931)
        (19.9203187250996, 40.65040650406504)
        (19.721115537848604, 40.40816326530612)
        (19.52191235059761, 40.66390041493776)
        (19.322709163346612, 40.416666666666664)
        (19.12350597609562, 40.67796610169492)
        (18.92430278884462, 40.94827586206897)
        (18.725099601593627, 40.692640692640694)
        (18.52589641434263, 40.43478260869565)
        (18.326693227091635, 40.174672489082965)
        (18.127490039840637, 40.44444444444444)
        (17.928286852589643, 40.723981900452486)
        (17.729083665338646, 40.45454545454545)
        (17.52988047808765, 41.1214953271028)
        (17.330677290836654, 40.845070422535215)
        (16.93227091633466, 40.476190476190474)
        (16.733067729083665, 40.77669902912621)
        (16.533864541832667, 40.487804878048784)
        (16.334661354581673, 41.41414141414141)
        (16.135458167330675, 41.53846153846154)
        (15.936254980079681, 42.32804232804233)
        (15.737051792828685, 42.02127659574468)
        (15.53784860557769, 41.711229946524064)
        (15.338645418326694, 42.07650273224044)
        (15.139442231075698, 41.75824175824176)
        (14.741035856573706, 41.340782122905026)
        (14.54183266932271, 41.47727272727273)
        (14.342629482071715, 41.14285714285714)
        (14.143426294820719, 43.03030303030303)
        (13.745019920318724, 42.592592592592595)
        (13.545816733067728, 42.2360248447205)
        (13.346613545816732, 42.675159235668794)
        (13.147410358565736, 42.857142857142854)
        (12.94820717131474, 42.48366013071895)
        (12.749003984063744, 42.10526315789473)
        (12.549800796812749, 42.281879194630875)
        (12.350597609561753, 41.891891891891895)
        (12.151394422310757, 42.65734265734265)
        (11.952191235059761, 42.5531914893617)
        (11.752988047808765, 43.06569343065693)
        (11.553784860557768, 43.93939393939394)
        (11.354581673306772, 43.51145038167939)
        (11.155378486055776, 43.07692307692308)
        (10.95617529880478, 42.63565891472868)
        (10.756972111553784, 42.1875)
        (10.557768924302788, 42.4)
        (10.358565737051793, 42.27642276422765)
        (10.159362549800797, 42.5)
        (9.9601593625498, 42.016806722689076)
        (9.760956175298805, 42.608695652173914)
        (9.56175298804781, 42.10526315789473)
        (9.362549800796813, 41.964285714285715)
        (9.163346613545817, 41.81818181818181)
        (8.964143426294822, 42.45283018867924)
        (8.764940239043826, 41.904761904761905)
        (8.565737051792828, 42.57425742574257)
        (8.366533864541832, 42.0)
        (8.167330677290837, 41.83673469387755)
        (7.968127490039841, 41.23711340206185)
        (7.768924302788845, 40.625)
        (7.569721115537849, 40.0)
        (7.370517928286853, 40.21739130434783)
        (7.171314741035857, 40.44943820224719)
        (6.97211155378486, 39.77272727272727)
        (6.772908366533864, 39.53488372093023)
        (6.573705179282868, 38.82352941176471)
        (6.374501992031872, 38.095238095238095)
        (6.175298804780876, 40.78947368421053)
        (5.9760956175298805, 44.11764705882353)
        (5.776892430278884, 45.3125)
        (5.577689243027888, 44.44444444444444)
        (5.378486055776892, 45.0)
        (5.179282868525896, 50.0)
        (4.780876494023905, 48.97959183673469)
        (4.581673306772909, 50.0)
        (4.382470119521913, 52.38095238095239)
        (4.183266932270916, 53.84615384615385)
        (3.9840637450199203, 54.054054054054056)
        (3.7848605577689245, 54.285714285714285)
        (3.5856573705179287, 56.25)
        (3.386454183266932, 56.666666666666664)
        (3.187250996015936, 55.172413793103445)
        (2.9880478087649402, 55.55555555555556)
        (2.788844621513944, 53.84615384615385)
        (2.589641434262948, 56.52173913043478)
        (2.3904382470119523, 57.14285714285714)
        (2.1912350597609564, 57.89473684210527)
        (1.9920318725099602, 66.66666666666666)
        (1.7928286852589643, 64.28571428571429)
        (1.593625498007968, 61.53846153846154)
        (1.394422310756972, 58.333333333333336)
        (1.1952191235059761, 54.54545454545454)
        (0.9960159362549801, 62.5)
        (0.796812749003984, 57.14285714285714)
        (0.796812749003984, 66.66666666666666)
        (0.5976095617529881, 60.0)
        (0.398406374501992, 50.0)
        (0.398406374501992, 66.66666666666666)
        (0.199203187250996, 50.0)
        (0.0, 100.0)
};
% Unigram
\addplot [draw=myyellow, line width=1.1pt] coordinates {
        (100.0, 12.776588151320487)
        (100.0, 12.794853466761975)
        (98.88268156424581, 12.670007158196134)
        (97.20670391061452, 12.56317689530686)
        (94.97206703910615, 12.67710663683818)
        (93.85474860335195, 12.56544502617801)
        (93.29608938547486, 12.680334092634777)
        (91.06145251396647, 12.5)
        (90.5027932960894, 12.607003891050583)
        (89.94413407821229, 12.70718232044199)
        (87.70949720670392, 12.837285363859364)
        (87.15083798882681, 12.956810631229235)
        (85.47486033519553, 12.846347607052897)
        (83.24022346368714, 12.745936698032507)
        (80.44692737430168, 12.620508326029798)
        (79.88826815642457, 12.756467439785906)
        (78.2122905027933, 12.556053811659194)
        (75.97765363128491, 12.307692307692308)
        (73.74301675977654, 12.199630314232902)
        (71.50837988826815, 12.075471698113208)
        (70.39106145251397, 11.909262759924385)
        (66.4804469273743, 11.68958742632613)
        (65.36312849162012, 11.794354838709678)
        (63.687150837988824, 11.62079510703364)
        (62.56983240223464, 11.727748691099476)
        (61.452513966480446, 11.840688912809473)
        (60.33519553072626, 11.650485436893204)
        (57.54189944134078, 11.495535714285714)
        (56.424581005586596, 11.361079865016873)
        (55.3072625698324, 11.25)
        (54.7486033519553, 11.36890951276102)
        (54.18994413407822, 11.729141475211609)
        (53.63128491620112, 12.045169385194479)
        (52.513966480446925, 11.883691529709228)
        (51.39664804469274, 11.7797695262484)
        (50.83798882681564, 11.926605504587156)
        (50.27932960893855, 12.064343163538874)
        (49.162011173184354, 11.875843454790823)
        (48.60335195530726, 12.049861495844876)
        (47.486033519553075, 12.160228898426324)
        (46.36871508379888, 11.99421965317919)
        (45.2513966480447, 11.756168359941945)
        (44.6927374301676, 11.627906976744185)
        (44.134078212290504, 11.738484398216938)
        (43.575418994413404, 11.981566820276496)
        (43.01675977653631, 11.846153846153847)
        (41.899441340782126, 12.155591572123177)
        (41.340782122905026, 12.271973466003317)
        (40.22346368715084, 12.060301507537687)
        (38.547486033519554, 11.794871794871794)
        (37.43016759776536, 11.591695501730104)
        (36.312849162011176, 11.403508771929824)
        (34.63687150837989, 11.272727272727273)
        (33.5195530726257, 10.968921389396709)
        (32.960893854748605, 11.090225563909774)
        (32.402234636871505, 10.984848484848484)
        (31.843575418994412, 11.242603550295858)
        (31.28491620111732, 11.642411642411643)
        (30.16759776536313, 11.440677966101696)
        (29.05027932960894, 11.23110151187905)
        (27.932960893854748, 10.869565217391305)
        (26.81564245810056, 10.983981693363845)
        (26.256983240223462, 10.87962962962963)
        (25.69832402234637, 10.74766355140187)
        (25.139664804469277, 10.869565217391305)
        (24.581005586592177, 10.679611650485436)
        (23.463687150837988, 10.44776119402985)
        (22.905027932960895, 10.25)
        (22.3463687150838, 10.050251256281408)
        (21.787709497206702, 10.182767624020887)
        (21.22905027932961, 10.079575596816976)
        (20.670391061452513, 9.840425531914894)
        (19.553072625698324, 10.23391812865497)
        (18.994413407821227, 11.724137931034482)
        (18.435754189944134, 12.043795620437956)
        (17.877094972067038, 11.851851851851853)
        (17.318435754189945, 12.4)
        (16.75977653631285, 12.875536480686694)
        (15.64245810055866, 12.173913043478262)
        (14.52513966480447, 12.322274881516588)
        (13.40782122905028, 11.483253588516746)
        (12.849162011173185, 11.616161616161616)
        (12.290502793296088, 11.76470588235294)
        (11.1731843575419, 11.299435028248588)
        (10.614525139664805, 10.795454545454545)
        (10.05586592178771, 10.285714285714285)
        (9.497206703910614, 10.059171597633137)
        (8.938547486033519, 10.884353741496598)
        (7.82122905027933, 9.655172413793103)
        (7.262569832402235, 10.743801652892563)
        (6.70391061452514, 11.428571428571429)
        (6.145251396648044, 15.942028985507244)
        (5.58659217877095, 14.705882352941178)
        (5.027932960893855, 13.846153846153847)
        (4.4692737430167595, 16.3265306122449)
        (3.910614525139665, 14.893617021276595)
        (3.35195530726257, 25.0)
        (2.793296089385475, 22.727272727272727)
        (2.2346368715083798, 21.052631578947366)
        (1.675977653631285, 23.076923076923077)
        (1.1173184357541899, 33.33333333333333)
        (0.0, 100.0)
};


==> figures/selfcheckgpt-factual.tex <==
% ours
\addplot [draw=mygreen, line width=1.1pt] coordinates {
  (100.0, 46.78787878787879)
  (68.39378238341969, 63.1578947368421)
  (67.35751295336787, 63.41463414634146)
  (64.76683937823834, 65.96306068601582)
  (64.24870466321244, 66.31016042780749)
  (63.47150259067358, 67.12328767123287)
  (62.95336787564767, 67.68802228412257)
  (62.69430051813472, 68.16901408450704)
  (61.917098445595855, 68.67816091954023)
  (61.398963730569946, 68.8953488372093)
  (60.362694300518136, 68.73156342182891)
  (60.10362694300518, 69.04761904761905)
  (59.84455958549223, 69.57831325301204)
  (59.58549222797927, 69.90881458966565)
  (59.32642487046632, 70.03058103975535)
  (58.80829015544041, 69.84615384615384)
  (57.77202072538861, 69.6875)
  (57.51295336787565, 70.70063694267516)
  (57.2538860103627, 70.83333333333334)
  (56.73575129533679, 71.56862745098039)
  (56.21761658031088, 71.38157894736842)
  (55.44041450777202, 72.05387205387206)
  (55.181347150259064, 72.6962457337884)
  (54.92227979274611, 73.10344827586206)
  (54.40414507772021, 73.68421052631578)
  (54.145077720207254, 74.11347517730496)
  (53.626943005181346, 75.0)
  (53.36787564766839, 75.18248175182481)
  (53.10880829015544, 75.64575645756457)
  (52.84974093264248, 75.8364312267658)
  (51.813471502590666, 76.04562737642586)
  (50.77720207253886, 76.26459143968872)
  (49.740932642487046, 75.8893280632411)
  (49.48186528497409, 76.09561752988047)
  (49.22279792746114, 76.61290322580645)
  (48.96373056994819, 76.82926829268293)
  (47.92746113989637, 77.08333333333334)
  (47.40932642487047, 76.89075630252101)
  (46.89119170984456, 76.69491525423729)
  (46.63212435233161, 76.92307692307693)
  (46.1139896373057, 77.05627705627705)
  (45.59585492227979, 77.19298245614034)
  (45.33678756476684, 77.09251101321586)
  (44.81865284974093, 77.92792792792793)
  (44.30051813471503, 77.72727272727272)
  (44.04145077720207, 78.70370370370371)
  (43.523316062176164, 78.50467289719626)
  (43.26424870466321, 79.14691943127961)
  (43.005181347150256, 79.42583732057416)
  (42.74611398963731, 79.71014492753623)
  (41.968911917098445, 79.41176470588235)
  (41.70984455958549, 79.70297029702971)
  (41.45077720207254, 80.0)
  (41.19170984455959, 79.89949748743719)
  (40.932642487046635, 80.20304568527918)
  (40.41450777202073, 80.82901554404145)
  (39.89637305699482, 80.6282722513089)
  (38.60103626943005, 81.86813186813187)
  (36.787564766839374, 83.52941176470588)
  (36.26943005181347, 83.33333333333334)
  (35.49222797927461, 85.09316770186336)
  (35.233160621761655, 85.53459119496856)
  (34.715025906735754, 85.35031847133759)
  (34.196891191709845, 85.16129032258064)
  (32.90155440414508, 84.66666666666667)
  (32.64248704663213, 85.13513513513513)
  (31.606217616580313, 84.72222222222221)
  (30.82901554404145, 85.0)
  (30.569948186528496, 85.5072463768116)
  (29.533678756476682, 85.07462686567165)
  (29.274611398963728, 85.60606060606061)
  (29.015544041450774, 85.49618320610686)
  (28.756476683937827, 85.38461538461539)
  (28.497409326424872, 85.9375)
  (27.979274611398964, 86.4)
  (27.72020725388601, 86.29032258064517)
  (27.202072538860104, 86.0655737704918)
  (26.165803108808287, 86.32478632478633)
  (25.647668393782386, 86.8421052631579)
  (25.38860103626943, 86.72566371681415)
  (24.61139896373057, 86.36363636363636)
  (24.093264248704664, 87.73584905660378)
  (23.316062176165804, 88.23529411764706)
  (23.05699481865285, 88.11881188118812)
  (21.761658031088082, 88.42105263157895)
  (21.502590673575128, 88.29787234042553)
  (20.207253886010363, 88.63636363636364)
  (18.65284974093264, 88.88888888888889)
  (17.616580310880828, 89.47368421052632)
  (17.098445595854923, 91.66666666666666)
  (16.83937823834197, 92.85714285714286)
  (16.580310880829018, 92.7536231884058)
  (16.06217616580311, 92.53731343283582)
  (15.803108808290157, 92.42424242424242)
  (15.544041450777202, 92.3076923076923)
  (14.766839378238341, 91.93548387096774)
  (14.248704663212436, 91.66666666666666)
  (13.989637305699482, 91.52542372881356)
  (12.953367875647666, 90.9090909090909)
  (12.694300518134716, 92.45283018867924)
  (12.435233160621761, 92.3076923076923)
  (11.917098445595855, 92.0)
  (11.139896373056994, 91.48936170212765)
  (10.621761658031089, 91.11111111111111)
  (9.844559585492227, 90.47619047619048)
  (9.067357512953368, 89.74358974358975)
  (0.0, 100.0)

};

% BertScore
\addplot [draw=myred, line width=1.1pt] coordinates {
  (100.0, 46.73123486682809)
  (100.0, 46.78787878787879)
  (99.74093264248705, 46.89403166869671)
  (99.48186528497409, 47.00122399020808)
  (99.22279792746113, 47.28395061728395)
  (98.96373056994818, 47.39454094292804)
  (98.70466321243524, 47.50623441396509)
  (98.44559585492227, 47.61904761904761)
  (98.18652849740933, 47.85353535353536)
  (97.40932642487047, 47.95918367346938)
  (97.15025906735751, 48.07692307692308)
  (96.6321243523316, 47.943444730077125)
  (95.85492227979275, 47.80361757105943)
  (95.59585492227978, 48.046875)
  (95.33678756476684, 48.167539267015705)
  (94.04145077720207, 48.01587301587302)
  (93.78238341968913, 48.138297872340424)
  (93.52331606217616, 48.26203208556149)
  (93.26424870466322, 48.38709677419355)
  (93.00518134715026, 48.77717391304348)
  (92.74611398963731, 48.90710382513661)
  (92.48704663212435, 49.03846153846153)
  (91.96891191709845, 49.16897506925208)
  (91.19170984455958, 49.299719887955185)
  (90.93264248704664, 49.436619718309856)
  (90.15544041450777, 49.29178470254957)
  (89.89637305699482, 49.50071326676177)
  (89.37823834196891, 49.35622317596567)
  (89.11917098445595, 49.49640287769784)
  (87.8238341968912, 49.34497816593886)
  (87.56476683937824, 49.487554904831626)
  (87.04663212435233, 49.63072378138848)
  (86.78756476683938, 49.77711738484398)
  (86.52849740932642, 49.92526158445441)
  (85.75129533678756, 50.07564296520424)
  (85.23316062176166, 50.229007633587784)
  (84.4559585492228, 50.38639876352396)
  (84.19689119170984, 51.02040816326531)
  (83.93782383419689, 51.347068145800314)
  (83.67875647668393, 51.68000000000001)
  (83.16062176165802, 51.52487961476726)
  (82.64248704663213, 51.368760064412236)
  (82.12435233160622, 51.54471544715447)
  (81.60621761658031, 51.386623164763456)
  (81.34715025906736, 51.64473684210527)
  (80.56994818652849, 51.49006622516556)
  (80.05181347150258, 51.67224080267558)
  (79.79274611398964, 51.85185185185185)
  (79.27461139896373, 51.95246179966044)
  (79.01554404145078, 52.13675213675214)
  (78.75647668393782, 52.323580034423415)
  (77.97927461139896, 52.16637781629117)
  (77.46113989637306, 52.27272727272727)
  (76.68393782383419, 52.112676056338024)
  (76.42487046632125, 52.584670231729056)
  (75.90673575129534, 52.41502683363149)
  (75.64766839378238, 52.51798561151079)
  (75.38860103626943, 52.62206148282098)
  (75.12953367875647, 52.72727272727272)
  (74.87046632124353, 52.833638025594155)
  (74.61139896373057, 52.94117647058824)
  (74.35233160621762, 53.04990757855823)
  (74.09326424870466, 53.159851301115246)
  (73.57512953367875, 52.98507462686567)
  (73.31606217616581, 53.09568480300187)
  (72.53886010362694, 52.93005671077504)
  (72.279792746114, 53.65384615384615)
  (71.50259067357513, 53.48837209302325)
  (71.24352331606218, 53.606237816764136)
  (70.98445595854922, 53.72549019607843)
  (70.46632124352331, 53.54330708661418)
  (70.20725388601036, 53.663366336633665)
  (69.68911917098445, 53.47912524850894)
  (69.17098445595855, 53.293413173652695)
  (68.9119170984456, 53.41365461847389)
  (68.65284974093264, 53.7525354969574)
  (68.13471502590673, 53.893442622950815)
  (67.87564766839378, 54.02061855670103)
  (67.35751295336787, 53.83022774327122)
  (66.83937823834198, 53.638253638253644)
  (66.06217616580311, 53.459119496855344)
  (65.80310880829016, 53.69978858350951)
  (65.5440414507772, 53.829787234042556)
  (64.76683937823834, 53.648068669527895)
  (64.24870466321244, 53.44827586206896)
  (63.98963730569949, 53.34773218142549)
  (63.730569948186535, 53.246753246753244)
  (63.47150259067358, 53.14533622559653)
  (63.212435233160626, 53.04347826086957)
  (62.95336787564767, 53.17286652078774)
  (62.69430051813472, 53.07017543859649)
  (62.43523316062176, 53.20088300220751)
  (62.17616580310881, 53.09734513274337)
  (61.917098445595855, 52.993348115299334)
  (61.6580310880829, 53.125)
  (60.880829015544045, 52.92792792792793)
  (60.62176165803109, 52.82167042889391)
  (60.362694300518136, 52.95454545454545)
  (60.10362694300518, 53.45622119815668)
  (59.84455958549223, 53.596287703016245)
  (59.58549222797927, 53.48837209302325)
  (58.80829015544041, 53.286384976525824)
  (58.549222797927456, 53.17647058823529)
  (58.2901554404145, 53.827751196172244)
  (58.03108808290155, 53.975903614457835)
  (57.77202072538861, 53.864734299516904)
  (57.51295336787565, 54.41176470588235)
  (57.2538860103627, 54.2997542997543)
  (56.994818652849744, 54.187192118226605)
  (56.73575129533679, 54.074074074074076)
  (56.476683937823836, 53.960396039603964)
  (56.21761658031088, 54.11471321695761)
  (55.95854922279793, 54.54545454545454)
  (55.69948186528497, 54.43037974683544)
  (55.44041450777202, 54.73145780051151)
  (55.181347150259064, 54.61538461538461)
  (54.92227979274611, 54.498714652956295)
  (54.66321243523316, 54.8051948051948)
  (54.40414507772021, 54.6875)
  (54.145077720207254, 54.85564304461942)
  (53.8860103626943, 54.736842105263165)
  (53.626943005181346, 54.61741424802111)
  (53.36787564766839, 54.78723404255319)
  (53.10880829015544, 54.666666666666664)
  (52.84974093264248, 54.98652291105122)
  (52.59067357512953, 55.16304347826087)
  (52.331606217616574, 55.04087193460491)
  (52.07253886010362, 55.219780219780226)
  (51.813471502590666, 55.4016620498615)
  (51.554404145077726, 56.056338028169016)
  (51.29533678756477, 56.25)
  (51.03626943005182, 56.12535612535613)
  (50.77720207253886, 56.00000000000001)
  (50.0, 55.78034682080924)
  (49.740932642487046, 55.97667638483965)
  (49.48186528497409, 55.84795321637427)
  (49.22279792746114, 55.718475073313776)
  (48.96373056994819, 55.917159763313606)
  (48.704663212435236, 55.78635014836796)
  (48.44559585492228, 55.98802395209581)
  (48.18652849740933, 55.85585585585585)
  (47.92746113989637, 56.060606060606055)
  (47.66839378238342, 55.92705167173252)
  (47.40932642487047, 55.79268292682927)
  (47.15025906735752, 55.65749235474006)
  (46.63212435233161, 55.55555555555556)
  (46.373056994818654, 55.417956656346746)
  (46.1139896373057, 55.27950310559007)
  (45.854922279792746, 55.140186915887845)
  (45.59585492227979, 55.34591194968554)
  (45.33678756476684, 55.55555555555556)
  (44.81865284974093, 55.44871794871795)
  (44.30051813471503, 55.33980582524271)
  (43.78238341968912, 55.22875816993464)
  (43.26424870466321, 55.115511551155116)
  (43.005181347150256, 54.966887417218544)
  (42.74611398963731, 54.81727574750831)
  (42.2279792746114, 54.69798657718121)
  (41.968911917098445, 54.54545454545454)
  (41.70984455958549, 54.391891891891895)
  (41.45077720207254, 54.794520547945204)
  (41.19170984455959, 55.208333333333336)
  (40.932642487046635, 55.052264808362374)
  (40.67357512953368, 55.673758865248224)
  (40.41450777202073, 56.72727272727273)
  (40.15544041450777, 56.56934306569343)
  (39.89637305699482, 56.41025641025641)
  (39.637305699481864, 56.25)
  (39.37823834196891, 56.92883895131086)
  (39.119170984455955, 56.766917293233085)
  (38.860103626943, 56.60377358490566)
  (38.60103626943005, 56.439393939393945)
  (38.082901554404145, 56.32183908045977)
  (37.82383419689119, 56.58914728682171)
  (37.30569948186528, 56.470588235294116)
  (37.04663212435233, 56.2992125984252)
  (36.787564766839374, 56.573705179282875)
  (36.52849740932643, 57.3170731707317)
  (36.01036269430052, 57.20164609053497)
  (35.751295336787564, 57.02479338842975)
  (35.49222797927461, 56.84647302904564)
  (35.233160621761655, 56.666666666666664)
  (34.97409326424871, 56.48535564853556)
  (34.715025906735754, 56.30252100840336)
  (34.196891191709845, 56.17021276595745)
  (33.93782383419689, 56.46551724137932)
  (33.67875647668394, 56.27705627705628)
  (33.160621761658035, 56.14035087719298)
  (32.90155440414508, 55.947136563876654)
  (32.64248704663213, 56.25)
  (32.12435233160622, 56.10859728506787)
  (31.865284974093267, 56.42201834862385)
  (31.606217616580313, 56.22119815668203)
  (31.34715025906736, 56.018518518518526)
  (31.088082901554404, 56.33802816901409)
  (30.82901554404145, 56.666666666666664)
  (30.569948186528496, 56.45933014354066)
  (30.05181347150259, 56.310679611650485)
  (29.792746113989637, 56.65024630541872)
  (29.533678756476682, 56.43564356435643)
  (29.274611398963728, 56.21890547263681)
  (29.015544041450774, 56.00000000000001)
  (28.756476683937827, 55.778894472361806)
  (28.497409326424872, 56.12244897959183)
  (28.238341968911918, 56.770833333333336)
  (27.979274611398964, 57.14285714285714)
  (27.72020725388601, 56.91489361702128)
  (27.202072538860104, 56.75675675675676)
  (26.94300518134715, 56.52173913043478)
  (26.683937823834196, 56.284153005464475)
  (26.42487046632124, 56.043956043956044)
  (25.906735751295333, 55.865921787709496)
  (25.647668393782386, 56.57142857142857)
  (25.38860103626943, 57.647058823529406)
  (25.129533678756477, 57.396449704142015)
  (24.870466321243523, 57.14285714285714)
  (24.61139896373057, 57.57575757575758)
  (24.352331606217618, 57.3170731707317)
  (24.093264248704664, 57.7639751552795)
  (23.83419689119171, 57.49999999999999)
  (23.316062176165804, 57.324840764331206)
  (23.05699481865285, 57.05128205128205)
  (22.797927461139896, 56.774193548387096)
  (22.53886010362694, 56.493506493506494)
  (22.279792746113987, 57.333333333333336)
  (22.020725388601036, 57.04697986577181)
  (21.761658031088082, 57.534246575342465)
  (21.502590673575128, 57.24137931034483)
  (21.243523316062177, 56.94444444444444)
  (20.984455958549223, 56.64335664335665)
  (20.72538860103627, 56.33802816901409)
  (20.207253886010363, 56.11510791366906)
  (19.94818652849741, 55.79710144927537)
  (19.4300518134715, 55.55555555555556)
  (18.911917098445596, 55.3030303030303)
  (18.65284974093264, 54.961832061068705)
  (18.393782383419687, 54.61538461538461)
  (17.875647668393782, 54.330708661417326)
  (17.616580310880828, 54.83870967741935)
  (17.357512953367877, 54.47154471544715)
  (17.098445595854923, 54.09836065573771)
  (16.580310880829018, 53.78151260504202)
  (16.06217616580311, 53.44827586206896)
  (15.803108808290157, 53.04347826086957)
  (15.544041450777202, 52.63157894736842)
  (15.284974093264248, 52.21238938053098)
  (14.766839378238341, 51.81818181818182)
  (14.507772020725387, 51.37614678899083)
  (14.248704663212436, 52.88461538461539)
  (13.989637305699482, 52.42718446601942)
  (13.730569948186528, 51.9607843137255)
  (13.471502590673575, 53.608247422680414)
  (12.953367875647666, 53.191489361702125)
  (12.435233160621761, 52.74725274725275)
  (12.176165803108809, 53.40909090909091)
  (11.658031088082902, 52.94117647058824)
  (11.398963730569948, 52.38095238095239)
  (11.139896373056994, 53.086419753086425)
  (10.880829015544041, 52.5)
  (10.621761658031089, 51.89873417721519)
  (10.362694300518134, 51.28205128205128)
  (10.103626943005182, 52.0)
  (9.844559585492227, 53.52112676056338)
  (9.585492227979273, 52.85714285714286)
  (9.067357512953368, 52.23880597014925)
  (8.808290155440414, 51.515151515151516)
  (8.549222797927461, 50.76923076923077)
  (8.290155440414509, 51.61290322580645)
  (8.031088082901555, 50.81967213114754)
  (7.772020725388601, 50.0)
  (7.512953367875648, 51.78571428571429)
  (7.253886010362693, 50.90909090909091)
  (6.994818652849741, 51.92307692307693)
  (6.476683937823833, 51.02040816326531)
  (5.958549222797927, 50.0)
  (5.699481865284974, 51.162790697674424)
  (5.4404145077720205, 52.5)
  (5.181347150259067, 51.28205128205128)
  (4.66321243523316, 50.0)
  (4.145077720207254, 48.484848484848484)
  (3.8860103626943006, 46.875)
  (3.6269430051813467, 46.666666666666664)
  (3.3678756476683938, 48.148148148148145)
  (3.1088082901554404, 46.15384615384615)
  (2.849740932642487, 44.0)
  (2.5906735751295336, 43.47826086956522)
  (2.33160621761658, 40.909090909090914)
  (2.072538860103627, 38.095238095238095)
  (1.8134715025906734, 41.17647058823529)
  (1.5544041450777202, 37.5)
  (1.2953367875647668, 35.714285714285715)
  (1.0362694300518136, 40.0)
  (0.7772020725388601, 50.0)
  (0.7772020725388601, 60.0)
  (0.7772020725388601, 75.0)
  (0.5181347150259068, 66.66666666666666)
  (0.2590673575129534, 50.0)
  (0.2590673575129534, 100.0)
  (0.0, 100.0)
};

% MQAG
\addplot [draw=myblue, line width=1.1pt] coordinates {
  (100.0, 46.73123486682809)
  (100.0, 46.78787878787879)
  (100.0, 46.84466019417476)
  (100.0, 46.901579586877276)
  (100.0, 46.95863746958637)
  (100.0, 47.01583434835566)
  (100.0, 47.073170731707314)
  (100.0, 47.13064713064713)
  (99.48186528497409, 47.00122399020808)
  (99.22279792746113, 47.10947109471095)
  (98.96373056994818, 47.21878862793572)
  (98.70466321243524, 47.329192546583855)
  (98.44559585492227, 47.44069912609238)
  (98.18652849740933, 47.553324968632374)
  (97.66839378238342, 47.661188369152974)
  (96.89119170984456, 47.522236340533674)
  (96.6321243523316, 47.63729246487867)
  (96.37305699481865, 47.753530166880616)
  (96.11398963730569, 47.87096774193548)
  (95.85492227979275, 47.98962386511025)
  (95.59585492227978, 48.109517601043024)
  (95.33678756476684, 48.741721854304636)
  (95.07772020725389, 48.8681757656458)
  (94.81865284974094, 49.59349593495935)
  (94.55958549222798, 49.72752043596731)
  (94.04145077720207, 49.862637362637365)
  (93.78238341968913, 50.0)
  (93.52331606217616, 50.208623087621696)
  (93.26424870466322, 50.42016806722689)
  (91.70984455958549, 50.57142857142857)
  (91.19170984455958, 50.429799426934096)
  (90.93264248704664, 50.649350649350644)
  (90.67357512953367, 50.872093023255815)
  (89.89637305699482, 50.73099415204678)
  (89.63730569948186, 50.882352941176464)
  (89.37823834196891, 51.33928571428571)
  (89.11917098445595, 51.49700598802395)
  (88.86010362694302, 51.6566265060241)
  (88.3419689119171, 51.82370820668692)
  (88.08290155440415, 52.06738131699847)
  (87.8238341968912, 52.72161741835147)
  (86.52849740932642, 52.59842519685039)
  (86.26943005181347, 52.85714285714286)
  (85.75129533678756, 52.959999999999994)
  (85.49222797927462, 53.14009661835749)
  (84.4559585492228, 53.008130081300806)
  (83.67875647668393, 53.125)
  (83.41968911917098, 53.57737104825291)
  (82.90155440414507, 53.42237061769616)
  (82.64248704663213, 53.70370370370371)
  (82.12435233160622, 53.82003395585738)
  (81.86528497409327, 53.92491467576792)
  (81.60621761658031, 54.03087478559176)
  (81.34715025906736, 54.325259515570934)
  (81.0880829015544, 54.434782608695656)
  (80.56994818652849, 54.56140350877193)
  (80.31088082901555, 54.673721340388006)
  (80.05181347150258, 54.78723404255319)
  (79.79274611398964, 55.00000000000001)
  (79.53367875647669, 55.31531531531532)
  (79.27461139896373, 55.839416058394164)
  (79.01554404145078, 55.96330275229357)
  (78.75647668393782, 56.08856088560885)
  (78.49740932642487, 56.21521335807051)
  (77.46113989637306, 56.09756097560976)
  (77.2020725388601, 56.22641509433962)
  (76.94300518134715, 56.35673624288425)
  (76.16580310880829, 56.21414913957935)
  (75.38860103626943, 56.395348837209305)
  (74.87046632124353, 56.22568093385214)
  (74.61139896373057, 56.470588235294116)
  (74.09326424870466, 56.63366336633663)
  (73.31606217616581, 56.4870259481038)
  (73.05699481865285, 56.62650602409639)
  (72.7979274611399, 57.46421267893661)
  (72.279792746114, 57.64462809917356)
  (71.76165803108809, 57.46887966804979)
  (71.24352331606218, 57.65199161425576)
  (70.20725388601036, 57.537154989384284)
  (69.68911917098445, 57.356076759061835)
  (69.17098445595855, 57.17344753747323)
  (68.65284974093264, 56.98924731182796)
  (68.39378238341969, 57.14285714285714)
  (68.13471502590673, 57.29847494553377)
  (67.87564766839378, 57.45614035087719)
  (67.35751295336787, 57.64966740576497)
  (67.09844559585493, 57.94183445190156)
  (66.83937823834198, 58.371040723981906)
  (66.32124352331607, 58.18181818181818)
  (66.06217616580311, 58.48623853211009)
  (65.80310880829016, 58.66050808314087)
  (65.28497409326425, 58.46867749419954)
  (65.02590673575129, 58.64485981308412)
  (64.76683937823834, 58.82352941176471)
  (63.98963730569949, 58.66983372921615)
  (63.730569948186535, 58.85167464114832)
  (62.95336787564767, 58.69565217391305)
  (62.69430051813472, 58.595641646489106)
  (62.43523316062176, 58.78048780487804)
  (62.17616580310881, 58.679706601467)
  (61.917098445595855, 58.57843137254902)
  (61.6580310880829, 59.20398009950249)
  (61.398963730569946, 59.10224438902743)
  (61.13989637305699, 59.44584382871536)
  (60.880829015544045, 59.34343434343434)
  (60.62176165803109, 59.24050632911393)
  (60.362694300518136, 59.43877551020408)
  (60.10362694300518, 59.6401028277635)
  (59.84455958549223, 60.0)
  (59.58549222797927, 59.895833333333336)
  (59.32642487046632, 60.10498687664042)
  (59.067357512953365, 60.317460317460316)
  (58.80829015544041, 60.53333333333333)
  (58.549222797927456, 60.42780748663101)
  (58.2901554404145, 60.32171581769437)
  (58.03108808290155, 60.215053763440864)
  (57.77202072538861, 60.1078167115903)
  (57.51295336787565, 60.0)
  (57.2538860103627, 59.891598915989164)
  (56.994818652849744, 59.78260869565217)
  (56.73575129533679, 60.0)
  (56.476683937823836, 60.724233983286915)
  (56.21761658031088, 60.614525139664806)
  (55.95854922279793, 61.18980169971672)
  (55.69948186528497, 61.42857142857143)
  (55.44041450777202, 61.31805157593123)
  (55.181347150259064, 61.206896551724135)
  (54.92227979274611, 61.09510086455331)
  (54.66321243523316, 60.982658959537574)
  (54.40414507772021, 60.86956521739131)
  (54.145077720207254, 61.111111111111114)
  (53.8860103626943, 60.997067448680355)
  (53.626943005181346, 60.882352941176464)
  (53.36787564766839, 60.766961651917406)
  (53.10880829015544, 61.011904761904766)
  (52.84974093264248, 60.895522388059696)
  (52.59067357512953, 61.14457831325302)
  (52.331606217616574, 61.027190332326285)
  (52.07253886010362, 61.46788990825688)
  (51.813471502590666, 61.34969325153374)
  (51.554404145077726, 61.99376947040498)
  (51.29533678756477, 62.264150943396224)
  (51.03626943005182, 62.14511041009464)
  (50.77720207253886, 62.0253164556962)
  (50.51813471502591, 61.904761904761905)
  (49.740932642487046, 61.7363344051447)
  (49.48186528497409, 61.61290322580645)
  (48.96373056994819, 61.76470588235294)
  (48.704663212435236, 62.04620462046204)
  (48.44559585492228, 62.54180602006689)
  (48.18652849740933, 62.41610738255034)
  (47.92746113989637, 62.2895622895623)
  (47.66839378238342, 62.79863481228669)
  (47.40932642487047, 63.10344827586207)
  (47.15025906735752, 62.9757785467128)
  (46.89119170984456, 63.286713286713294)
  (46.373056994818654, 63.47517730496454)
  (46.1139896373057, 63.799283154121866)
  (45.854922279792746, 63.66906474820144)
  (45.07772020725388, 63.503649635036496)
  (44.81865284974093, 63.837638376383765)
  (44.559585492227974, 63.94052044609665)
  (44.30051813471503, 64.04494382022472)
  (44.04145077720207, 63.90977443609023)
  (43.78238341968912, 63.77358490566037)
  (43.523316062176164, 64.36781609195403)
  (43.26424870466321, 64.23076923076924)
  (43.005181347150256, 64.0926640926641)
  (42.74611398963731, 64.96062992125984)
  (42.487046632124354, 64.82213438735178)
  (42.2279792746114, 64.68253968253968)
  (41.968911917098445, 64.5418326693227)
  (41.70984455958549, 64.4)
  (41.45077720207254, 64.2570281124498)
  (41.19170984455959, 64.11290322580645)
  (40.932642487046635, 63.96761133603239)
  (40.67357512953368, 63.82113821138211)
  (40.41450777202073, 63.6734693877551)
  (40.15544041450777, 63.52459016393443)
  (39.89637305699482, 63.63636363636363)
  (39.637305699481864, 63.48547717842323)
  (39.37823834196891, 63.33333333333333)
  (39.119170984455955, 63.71308016877637)
  (38.860103626943, 63.559322033898304)
  (38.60103626943005, 65.06550218340611)
  (38.34196891191709, 64.91228070175438)
  (38.082901554404145, 64.75770925110133)
  (37.82383419689119, 65.17857142857143)
  (37.56476683937824, 65.02242152466367)
  (37.30569948186528, 65.15837104072398)
  (37.04663212435233, 65.0)
  (36.787564766839374, 66.04651162790698)
  (36.52849740932643, 65.88785046728972)
  (36.26943005181347, 65.72769953051643)
  (36.01036269430052, 66.19047619047619)
  (35.751295336787564, 66.34615384615384)
  (35.49222797927461, 66.18357487922705)
  (35.233160621761655, 66.01941747572816)
  (34.97409326424871, 65.85365853658537)
  (34.715025906735754, 67.0)
  (34.4559585492228, 66.83417085427136)
  (34.196891191709845, 66.66666666666666)
  (33.93782383419689, 66.83673469387756)
  (33.67875647668394, 67.0103092783505)
  (33.41968911917099, 69.35483870967742)
  (33.160621761658035, 69.1891891891892)
  (32.90155440414508, 69.02173913043478)
  (32.64248704663213, 68.85245901639344)
  (32.38341968911917, 68.68131868131869)
  (32.12435233160622, 68.50828729281768)
  (31.865284974093267, 68.33333333333333)
  (31.606217616580313, 69.31818181818183)
  (31.34715025906736, 69.14285714285714)
  (31.088082901554404, 69.36416184971098)
  (30.82901554404145, 69.5906432748538)
  (30.569948186528496, 69.41176470588235)
  (30.310880829015545, 69.23076923076923)
  (30.05181347150259, 69.46107784431138)
  (29.792746113989637, 69.27710843373494)
  (29.533678756476682, 69.0909090909091)
  (29.274611398963728, 70.1863354037267)
  (29.015544041450774, 71.3375796178344)
  (28.756476683937827, 71.15384615384616)
  (28.497409326424872, 70.96774193548387)
  (28.238341968911918, 71.24183006535948)
  (27.979274611398964, 71.05263157894737)
  (27.72020725388601, 71.33333333333334)
  (27.461139896373055, 72.10884353741497)
  (27.202072538860104, 71.91780821917808)
  (26.94300518134715, 72.72727272727273)
  (26.683937823834196, 72.53521126760563)
  (26.42487046632124, 72.3404255319149)
  (26.165803108808287, 72.14285714285714)
  (25.906735751295333, 71.94244604316546)
  (25.647668393782386, 71.73913043478261)
  (25.38860103626943, 71.53284671532847)
  (25.129533678756477, 71.85185185185186)
  (24.870466321243523, 73.2824427480916)
  (24.61139896373057, 74.21875)
  (24.352331606217618, 74.01574803149606)
  (24.093264248704664, 74.4)
  (23.83419689119171, 74.79674796747967)
  (23.57512953367876, 74.59016393442623)
  (23.316062176165804, 74.3801652892562)
  (23.05699481865285, 74.16666666666667)
  (22.797927461139896, 73.94957983193278)
  (22.53886010362694, 74.35897435897436)
  (22.279792746113987, 74.13793103448276)
  (22.020725388601036, 73.91304347826086)
  (21.761658031088082, 73.68421052631578)
  (21.502590673575128, 73.45132743362832)
  (21.243523316062177, 77.35849056603774)
  (20.984455958549223, 77.14285714285715)
  (20.72538860103627, 76.92307692307693)
  (20.466321243523318, 76.69902912621359)
  (20.207253886010363, 76.47058823529412)
  (19.94818652849741, 76.23762376237624)
  (19.689119170984455, 76.0)
  (19.4300518134715, 75.75757575757575)
  (19.170984455958546, 75.51020408163265)
  (18.911917098445596, 76.04166666666666)
  (18.65284974093264, 76.59574468085107)
  (18.393782383419687, 76.34408602150538)
  (18.134715025906736, 76.08695652173914)
  (17.875647668393782, 75.82417582417582)
  (17.616580310880828, 75.55555555555556)
  (17.357512953367877, 75.28089887640449)
  (17.098445595854923, 75.0)
  (16.83937823834197, 74.71264367816092)
  (16.580310880829018, 75.29411764705883)
  (16.321243523316063, 75.0)
  (16.06217616580311, 76.5432098765432)
  (15.803108808290157, 76.25)
  (15.544041450777202, 75.9493670886076)
  (15.284974093264248, 75.64102564102564)
  (15.025906735751295, 75.32467532467533)
  (14.766839378238341, 75.0)
  (14.507772020725387, 74.66666666666667)
  (14.248704663212436, 74.32432432432432)
  (13.989637305699482, 76.05633802816901)
  (13.730569948186528, 76.81159420289855)
  (13.471502590673575, 76.47058823529412)
  (13.21243523316062, 77.27272727272727)
  (12.953367875647666, 76.92307692307693)
  (12.694300518134716, 77.77777777777779)
  (12.435233160621761, 77.41935483870968)
  (12.176165803108809, 78.33333333333333)
  (11.917098445595855, 77.96610169491525)
  (11.658031088082902, 78.94736842105263)
  (11.398963730569948, 78.57142857142857)
  (11.139896373056994, 78.18181818181819)
  (10.880829015544041, 77.77777777777779)
  (10.621761658031089, 77.35849056603774)
  (10.362694300518134, 76.92307692307693)
  (10.103626943005182, 76.47058823529412)
  (9.844559585492227, 76.0)
  (9.585492227979273, 75.51020408163265)
  (9.32642487046632, 75.0)
  (9.067357512953368, 74.46808510638297)
  (8.808290155440414, 73.91304347826086)
  (8.549222797927461, 75.0)
  (8.290155440414509, 74.4186046511628)
  (8.031088082901555, 77.5)
  (7.772020725388601, 76.92307692307693)
  (7.512953367875648, 78.37837837837837)
  (7.253886010362693, 77.77777777777779)
  (6.994818652849741, 77.14285714285715)
  (6.7357512953367875, 76.47058823529412)
  (6.476683937823833, 75.75757575757575)
  (6.217616580310881, 77.41935483870968)
  (5.958549222797927, 76.66666666666667)
  (5.699481865284974, 75.86206896551724)
  (5.4404145077720205, 75.0)
  (5.181347150259067, 80.0)
  (4.922279792746114, 82.6086956521739)
  (4.66321243523316, 81.81818181818183)
  (4.404145077720207, 80.95238095238095)
  (4.145077720207254, 88.88888888888889)
  (3.8860103626943006, 88.23529411764706)
  (3.6269430051813467, 87.5)
  (3.3678756476683938, 86.66666666666667)
  (3.1088082901554404, 85.71428571428571)
  (2.849740932642487, 84.61538461538461)
  (2.5906735751295336, 83.33333333333334)
  (2.33160621761658, 81.81818181818183)
  (2.072538860103627, 80.0)
  (1.8134715025906734, 77.77777777777779)
  (1.5544041450777202, 75.0)
  (1.2953367875647668, 71.42857142857143)
  (1.0362694300518136, 80.0)
  (0.7772020725388601, 75.0)
  (0.5181347150259068, 66.66666666666666)
  (0.2590673575129534, 50.0)
  (0.2590673575129534, 100.0)
  (0.0, 100.0)
};

% Unigram AVG
\addplot [draw=myyellow, line width=1.1pt] coordinates {
  (100.0, 49.87893462469734)
  (100.0, 49.93939393939394)
  (100.0, 50.0)
  (100.0, 50.06075334143378)
  (99.75728155339806, 50.18315018315018)
  (99.51456310679612, 50.306748466257666)
  (98.54368932038835, 50.43478260869565)
  (98.30097087378641, 50.625)
  (98.05825242718447, 50.753768844221106)
  (97.81553398058253, 50.88383838383839)
  (97.33009708737865, 50.75949367088608)
  (97.0873786407767, 51.02040816326531)
  (96.84466019417476, 51.153846153846146)
  (96.60194174757282, 51.28865979381443)
  (96.35922330097088, 51.42487046632125)
  (96.11650485436894, 51.5625)
  (95.63106796116504, 51.43603133159269)
  (95.14563106796116, 51.30890052356021)
  (94.90291262135922, 51.44736842105263)
  (94.1747572815534, 51.59574468085106)
  (92.96116504854369, 51.47849462365591)
  (92.47572815533981, 51.6260162601626)
  (91.50485436893204, 51.502732240437155)
  (91.01941747572816, 51.369863013698634)
  (90.53398058252428, 51.51933701657458)
  (90.0485436893204, 51.38504155124654)
  (88.59223300970875, 51.26404494382022)
  (88.3495145631068, 51.41242937853108)
  (88.10679611650485, 51.5625)
  (87.62135922330097, 51.42450142450142)
  (87.37864077669903, 51.57593123209169)
  (87.13592233009709, 51.72910662824207)
  (86.89320388349515, 51.8840579710145)
  (86.6504854368932, 52.11678832116788)
  (86.16504854368931, 51.97657393850659)
  (85.19417475728154, 51.8463810930576)
  (84.70873786407766, 51.70370370370371)
  (84.22330097087378, 51.56017830609212)
  (83.7378640776699, 51.41579731743666)
  (83.49514563106796, 51.80722891566265)
  (83.25242718446601, 51.96969696969697)
  (83.00970873786407, 52.13414634146341)
  (82.52427184466019, 51.98776758409785)
  (81.79611650485437, 51.84615384615384)
  (81.55339805825243, 52.012383900928796)
  (80.33980582524272, 51.88087774294671)
  (79.85436893203884, 51.729559748427675)
  (79.12621359223301, 51.58227848101266)
  (78.39805825242718, 51.76282051282052)
  (77.66990291262135, 51.86385737439222)
  (76.94174757281553, 51.71288743882545)
  (76.2135922330097, 51.55993431855501)
  (75.72815533980582, 51.40032948929159)
  (75.48543689320388, 51.575456053067995)
  (74.75728155339806, 51.41903171953256)
  (74.02912621359224, 51.26050420168067)
  (73.05825242718447, 51.103565365025474)
  (72.81553398058253, 51.28205128205128)
  (72.33009708737865, 51.114922813036024)
  (71.84466019417476, 50.94664371772806)
  (71.60194174757282, 51.12651646447141)
  (71.11650485436894, 51.31348511383538)
  (70.3883495145631, 51.41843971631206)
  (69.90291262135922, 51.52057245080501)
  (69.66019417475728, 51.711711711711715)
  (69.1747572815534, 51.81818181818182)
  (68.93203883495146, 51.91956124314442)
  (68.68932038834951, 52.117863720073665)
  (68.44660194174757, 52.22222222222223)
  (68.20388349514563, 52.327746741154556)
  (67.96116504854369, 52.43445692883895)
  (67.23300970873787, 52.264150943396224)
  (66.99029126213593, 52.47148288973384)
  (66.50485436893204, 52.5911708253359)
  (66.01941747572816, 52.408477842003855)
  (65.77669902912622, 52.51937984496124)
  (65.29126213592234, 52.33463035019456)
  (65.0485436893204, 52.54901960784314)
  (64.80582524271846, 52.76679841897233)
  (64.32038834951457, 52.57936507936508)
  (63.834951456310684, 52.39043824701195)
  (63.59223300970874, 52.505010020040075)
  (63.10679611650486, 52.31388329979879)
  (61.89320388349514, 52.14723926380368)
  (61.6504854368932, 52.2633744855967)
  (61.165048543689316, 52.066115702479344)
  (60.679611650485434, 52.19206680584551)
  (60.43689320388349, 52.3109243697479)
  (60.19417475728155, 52.21052631578947)
  (59.95145631067961, 52.4416135881104)
  (59.70873786407766, 52.56410256410257)
  (59.46601941747572, 52.46252676659529)
  (59.22330097087378, 52.36051502145923)
  (58.98058252427184, 52.25806451612903)
  (58.7378640776699, 52.38095238095239)
  (58.495145631067956, 52.27765726681128)
  (58.252427184466015, 52.40174672489083)
  (58.009708737864074, 52.52747252747253)
  (57.76699029126213, 52.77161862527716)
  (57.52427184466019, 53.139013452914796)
  (57.28155339805825, 53.51473922902494)
  (56.79611650485437, 53.669724770642205)
  (56.55339805825243, 53.5632183908046)
  (56.310679611650485, 53.45622119815668)
  (56.067961165048544, 53.34872979214781)
  (55.8252427184466, 53.73831775700935)
  (55.09708737864077, 53.5377358490566)
  (54.36893203883495, 53.333333333333336)
  (54.12621359223301, 53.47721822541966)
  (53.883495145631066, 53.62318840579711)
  (53.640776699029125, 53.771289537712896)
  (53.398058252427184, 53.65853658536586)
  (53.15533980582524, 53.54523227383863)
  (52.42718446601942, 53.333333333333336)
  (52.18446601941748, 53.75)
  (51.94174757281553, 53.63408521303258)
  (51.69902912621359, 53.92405063291139)
  (51.45631067961165, 53.80710659898477)
  (51.213592233009706, 53.68956743002544)
  (50.970873786407765, 53.84615384615385)
  (50.728155339805824, 53.72750642673522)
  (50.48543689320388, 53.608247422680414)
  (50.24271844660194, 53.76623376623376)
  (50.0, 53.645833333333336)
  (49.75728155339806, 53.805774278215225)
  (49.51456310679612, 53.68421052631579)
  (49.271844660194176, 53.84615384615385)
  (49.029126213592235, 54.01069518716578)
  (48.786407766990294, 54.17789757412399)
  (48.54368932038835, 54.347826086956516)
  (48.30097087378641, 54.223433242506815)
  (48.05825242718447, 54.09836065573771)
  (47.81553398058252, 53.97260273972603)
  (47.57281553398058, 53.84615384615385)
  (47.33009708737864, 53.71900826446281)
  (47.0873786407767, 53.888888888888886)
  (46.84466019417476, 53.760445682451255)
  (46.601941747572816, 53.63128491620112)
  (46.359223300970875, 53.80281690140845)
  (45.87378640776699, 53.69318181818182)
  (45.63106796116505, 54.02298850574713)
  (45.14563106796117, 53.91304347826087)
  (44.90291262135923, 53.779069767441854)
  (44.66019417475729, 53.64431486880466)
  (44.417475728155345, 53.50877192982456)
  (44.1747572815534, 53.3724340175953)
  (43.932038834951456, 53.23529411764706)
  (43.689320388349515, 53.09734513274337)
  (43.44660194174757, 52.95857988165681)
  (43.203883495145625, 53.13432835820896)
  (42.961165048543684, 52.99401197604791)
  (42.71844660194174, 52.85285285285285)
  (42.4757281553398, 52.71084337349398)
  (42.23300970873786, 52.88753799392097)
  (41.99029126213592, 53.06748466257669)
  (41.50485436893204, 52.94117647058824)
  (41.262135922330096, 52.79503105590062)
  (41.019417475728154, 52.64797507788161)
  (40.77669902912621, 52.5)
  (40.53398058252427, 52.6813880126183)
  (40.29126213592233, 52.53164556962025)
  (40.04854368932039, 52.38095238095239)
  (39.80582524271845, 52.903225806451616)
  (39.32038834951456, 52.76872964169381)
  (39.07766990291262, 52.960526315789465)
  (38.83495145631068, 53.156146179402)
  (38.592233009708735, 53.535353535353536)
  (38.349514563106794, 53.92491467576792)
  (38.10679611650485, 54.137931034482754)
  (37.86407766990291, 54.35540069686411)
  (37.62135922330097, 54.1958041958042)
  (37.37864077669903, 54.03508771929825)
  (37.13592233009709, 54.25531914893617)
  (36.89320388349515, 54.092526690391466)
  (36.407766990291265, 53.956834532374096)
  (36.16504854368932, 54.379562043795616)
  (35.67961165048544, 54.24354243542435)
  (35.43689320388349, 54.47761194029851)
  (35.19417475728155, 54.30711610486891)
  (34.95145631067961, 54.13533834586466)
  (34.70873786407767, 53.9622641509434)
  (34.46601941747573, 53.78787878787878)
  (34.22330097087379, 54.440154440154444)
  (33.980582524271846, 54.263565891472865)
  (33.737864077669904, 54.509803921568626)
  (33.49514563106796, 54.330708661417326)
  (33.25242718446602, 54.1501976284585)
  (33.00970873786408, 53.96825396825397)
  (32.76699029126214, 53.78486055776892)
  (32.5242718446602, 54.03225806451613)
  (32.28155339805826, 54.285714285714285)
  (32.038834951456316, 54.09836065573771)
  (31.55339805825243, 53.941908713692946)
  (31.31067961165049, 53.75)
  (31.06796116504854, 54.008438818565395)
  (30.8252427184466, 53.813559322033896)
  (30.582524271844658, 54.310344827586206)
  (30.339805825242717, 54.824561403508774)
  (30.097087378640776, 54.62555066079295)
  (29.85436893203883, 54.424778761061944)
  (29.61165048543689, 54.22222222222223)
  (29.126213592233007, 54.054054054054056)
  (28.640776699029125, 53.88127853881278)
  (28.398058252427184, 53.669724770642205)
  (28.155339805825243, 53.95348837209303)
  (27.9126213592233, 53.73831775700935)
  (27.427184466019416, 53.55450236966824)
  (27.184466019417474, 53.333333333333336)
  (26.941747572815533, 53.62318840579711)
  (26.699029126213592, 53.398058252427184)
  (26.45631067961165, 53.170731707317074)
  (25.970873786407765, 52.97029702970298)
  (25.728155339805824, 54.08163265306123)
  (25.485436893203882, 53.84615384615385)
  (25.24271844660194, 53.608247422680414)
  (25.0, 53.36787564766839)
  (24.75728155339806, 53.125)
  (24.514563106796118, 54.3010752688172)
  (24.271844660194176, 55.55555555555556)
  (24.029126213592235, 55.3072625698324)
  (23.78640776699029, 55.0561797752809)
  (23.54368932038835, 54.80225988700565)
  (23.300970873786408, 54.54545454545454)
  (23.058252427184467, 54.285714285714285)
  (22.815533980582526, 54.65116279069767)
  (22.572815533980584, 54.385964912280706)
  (22.0873786407767, 54.166666666666664)
  (21.844660194174757, 54.54545454545454)
  (21.601941747572813, 55.27950310559007)
  (21.35922330097087, 55.00000000000001)
  (21.11650485436893, 54.71698113207547)
  (20.87378640776699, 55.12820512820513)
  (20.388349514563107, 54.90196078431373)
  (20.145631067961165, 55.333333333333336)
  (19.902912621359224, 55.78231292517006)
  (19.66019417475728, 55.47945205479452)
  (19.41747572815534, 55.172413793103445)
  (19.174757281553397, 54.861111111111114)
  (18.932038834951456, 56.11510791366906)
  (18.689320388349515, 55.79710144927537)
  (18.446601941747574, 55.47445255474452)
  (18.203883495145632, 55.14705882352941)
  (17.96116504854369, 54.81481481481482)
  (17.718446601941746, 54.47761194029851)
  (17.475728155339805, 54.13533834586466)
  (17.233009708737864, 53.78787878787878)
  (16.990291262135923, 54.263565891472865)
  (16.74757281553398, 53.90625)
  (16.50485436893204, 53.54330708661418)
  (16.2621359223301, 53.17460317460318)
  (15.776699029126215, 52.84552845528455)
  (15.53398058252427, 53.333333333333336)
  (15.291262135922329, 52.94117647058824)
  (14.805825242718445, 52.58620689655172)
  (14.563106796116504, 54.054054054054056)
  (14.320388349514563, 53.63636363636364)
  (13.834951456310678, 53.271028037383175)
  (13.592233009708737, 53.84615384615385)
  (13.349514563106796, 53.398058252427184)
  (13.106796116504855, 52.94117647058824)
  (12.864077669902912, 52.475247524752476)
  (12.62135922330097, 52.0)
  (12.37864077669903, 53.68421052631579)
  (12.135922330097088, 56.81818181818182)
  (11.893203883495145, 56.32183908045977)
  (11.650485436893204, 55.81395348837209)
  (11.407766990291263, 55.294117647058826)
  (11.165048543689322, 54.761904761904766)
  (10.922330097087379, 54.21686746987952)
  (10.679611650485436, 53.65853658536586)
  (10.436893203883495, 53.086419753086425)
  (9.951456310679612, 52.56410256410257)
  (9.70873786407767, 51.94805194805194)
  (9.466019417475728, 52.702702702702695)
  (9.223300970873787, 52.054794520547944)
  (8.980582524271846, 52.85714285714286)
  (8.737864077669903, 52.17391304347826)
  (8.495145631067961, 51.470588235294116)
  (8.25242718446602, 50.74626865671642)
  (8.009708737864079, 50.0)
  (7.766990291262135, 49.23076923076923)
  (7.281553398058252, 48.38709677419355)
  (7.038834951456311, 47.540983606557376)
  (6.796116504854369, 50.0)
  (6.553398058252427, 49.09090909090909)
  (6.310679611650485, 48.148148148148145)
  (6.067961165048544, 47.16981132075472)
  (5.825242718446602, 48.0)
  (5.582524271844661, 46.93877551020408)
  (5.339805825242718, 51.162790697674424)
  (4.854368932038835, 50.0)
  (4.611650485436893, 48.717948717948715)
  (4.12621359223301, 47.22222222222222)
  (3.8834951456310676, 48.484848484848484)
  (3.640776699029126, 46.875)
  (3.3980582524271843, 46.666666666666664)
  (3.1553398058252426, 44.827586206896555)
  (2.912621359223301, 44.44444444444444)
  (2.669902912621359, 47.82608695652174)
  (2.4271844660194173, 45.45454545454545)
  (2.1844660194174756, 56.25)
  (1.9417475728155338, 53.333333333333336)
  (1.6990291262135921, 53.84615384615385)
  (1.4563106796116505, 50.0)
  (1.2135922330097086, 45.45454545454545)
  (0.9708737864077669, 44.44444444444444)
  (0.7281553398058253, 37.5)
  (0.48543689320388345, 28.57142857142857)
  (0.48543689320388345, 33.33333333333333)
  (0.48543689320388345, 40.0)
  (0.48543689320388345, 50.0)
  (0.48543689320388345, 66.66666666666666)
  (0.24271844660194172, 50.0)
  (0.0, 100.0)
};
